Bridging the Semantic Gap with SQL Query Logs in Natural Language Interfaces to Databases

A critical challenge in constructing a natural language interface to database (NLIDB) is bridging the semantic gap between a natural language query (NLQ) and the underlying data. Two specific ways this challenge exhibits itself is through keyword mapping and join path inference. Keyword mapping is the task of mapping individual keywords in the original NLQ to database elements (such as relations, attributes or values). It is challenging due to the ambiguity in mapping the user's mental model and diction to the schema definition and contents of the underlying database. Join path inference is the process of selecting the relations and join conditions in the FROM clause of the final SQL query, and is difficult because NLIDB users lack the knowledge of the database schema or SQL and therefore cannot explicitly specify the intermediate tables and joins needed to construct a final SQL query. In this paper, we propose leveraging information from the SQL query log of a database to enhance the performance of existing NLIDBs with respect to these challenges. We present a system Templar that can be used to augment existing NLIDBs. Our extensive experimental evaluation demonstrates the effectiveness of our approach, leading up to 138% improvement in top-1 accuracy in existing NLIDBs by leveraging SQL query log information.

==> challenges.tex <==
% !TEX root = ms.tex

\section{Implementation Challenges}
\label{sec:challenges}

We implemented the ideas described above in a system called \system. While most of the implementation was straightforward, there were a couple of challenges. Here, we detail two specific implementation challenges we faced: one for keyword mapping and the other for join path inference.

\subsection{Handling Pairs}
\label{sec:pair}

One challenge in the process of keyword mapping is handling \textsf{Pair}-type query fragments. A \textsf{Pair} occurs when a single keyword maps to both a projection and predicate simultaneously. Consider the following NLQ on the schema in Figure~\ref{fig:mas}:

\begin{example}
Find the number of John Does at University X.
\end{example}

The keyword {\em John Does} should simultaneously yield the projection \texttt{SELECT COUNT(author.id)} and the predicate \texttt{author.name = 'John Doe'} to construct the correct query:

\begin{verbatim}
SELECT COUNT(author.aid)
FROM author a, organization o
WHERE author.name = 'John Doe'
  AND organization.name = 'University X'
  AND author.oid = organization.oid
\end{verbatim}

Existing parsers in NLIDBs can detect a \textsf{Pair} mapping when the keyword implies a projection yet represents an attribute value instead of an attribute name. For example, with the parsing strategy in NaLIR~\cite{li:nalir}, if the direct child of a command token (\eg\ {\em return}, {\em find}, {\em retrieve}, \etc) node is referring to an attribute value (\ie\ {\em John Does}, instead of an attribute name such as {\em authors}), this indicates that the keyword should be mapped to a \textsf{Pair}.

To facilitate these \textsf{Pair} structures, \system\ requires a {\em paired attribute} (Line \ref{algline:pairedattr}) be annotated on the schema for each non-key (\ie\ neither a foreign nor a primary key) attribute in $D$.

\begin{definition}[Paired Attribute]
A paired attribute for attribute $\alpha$ is an attribute $\alpha_\textit{pair}$ that should be projected in conjunction with a predicate of $\alpha$ when forming a \textsf{Pair}.
\end{definition}

\input{tables/pair}

By default, the paired attribute for any attribute will be its relation's primary key, as in the example above, where \texttt{author.aid} is the paired attribute for \texttt{author.name}. Some schemas, however, require manual annotation of paired attributes across different relations. For example, consider that we add a relation named \texttt{position} to the schema in Figure~\ref{fig:mas}, with two attributes as shown in Table~\ref{tab:pair}. If the user then issued the NLQ:

\begin{example}
Find all professors at University X.
\end{example}

The token {\em professors} corresponds to the value {\em Professor} of the \texttt{position.name} attribute, and the intent of this query is to return the professors' \texttt{author.name} values:

\begin{verbatim}
SELECT DISTINCT author.name
FROM author a, position p
WHERE position.name = 'Professor'
  AND author.aid = position.aid
\end{verbatim}

The paired attribute annotations on the schema allow us to successfully produce the correct projection.

\begin{figure}[t]
\centering
\subfloat[Before fork.]{
  \includegraphics[clip,width=0.32\columnwidth]{figs/prefork.pdf}
  \label{fig:prefork}
}\qquad%
\subfloat[After fork.]{
  \includegraphics[clip,width=0.51\columnwidth]{figs/postfork.pdf}
  \label{fig:postfork}
}
\caption{A simplified overview of a schema graph fork for self-joins.}
\label{fig:fork}
\vspace{-0.4cm}
\end{figure}

\subsection{Self-Joins}

A challenge arises during join path inference when the same attribute is included multiple times in the bag $B_D$ for a SQL translation. Due to the peculiarities of SQL, these situations require that our resulting join path include multiple instances of the same relation, resulting in a {\em self-join}. For example, in an NLQ for the academic database, {\em Find papers written by both John Doe and Jane Doe}, {\em John Doe} and {\em Jane Doe} both refer to attribute \texttt{author.name}. The correct SQL output for this NLQ is:

\begin{verbatim}
SELECT p.title
FROM author a1, author a2, publication p,
  writes w1, writes w2
WHERE a1.name = 'John Doe' AND a2.name = 'Jane Doe'
  AND a1.aid = w1.aid AND a2.aid = w2.aid
  AND p.pid = w1.pid AND p.pid = w2.pid
\end{verbatim}

\input{algs/fork}

For these situations, we ``fork'' the schema graph, as shown (with some attribute vertices and edges removed for simplicity) in Figure~\ref{fig:fork}, in order to account for the necessary vertices for a join path containing a self-join.

Algorithm~\ref{alg:fork} describes the process of forking the schema graph $G_s$ in more detail, given an attribute vertex $v$ that has been referenced multiple times. Two mirrored stacks $v_\textit{old}$ and $v_\textit{new}$ are used to track progress for the original graph and the new fork of the graph, respectively. We first clone the attribute vertex $v$ and add it to $G_s$ (Line \ref{algline:clone}). We repeatedly pop the top of each stack, and find all vertices $v_\textit{conn}$ that are connected to the current existing vertex $v_\textit{old}$. We clone each $v_\textit{conn}$ and the edge connecting it to $v_\textit{old}$, then add both to the schema graph and continue traversal (Lines \ref{algline:startfork}-\ref{algline:endfork}). We terminate the forking process when we reach a FK-PK join edge in the direction {\em from} $v_\textit{old}$ {\em to} $v_\textit{conn}$ (Line \ref{algline:termfork}). For $d$ duplicate references to an attribute vertex $v$, \textsc{Fork} is executed $d-1$ times to create a fork for each duplicate reference.

